From Physical to Cyber: Escalating Protection for Personalized Auto Insurance

Nowadays, auto insurance companies set personalized insurance rate based on data gathered directly from their customers' cars. In this paper, we show such a personalized insurance mechanism -- wildly adopted by many auto insurance companies -- is vulnerable to exploit. In particular, we demonstrate that an adversary can leverage off-the-shelf hardware to manipulate the data to the device that collects drivers' habits for insurance rate customization and obtain a fraudulent insurance discount. In response to this type of attack, we also propose a defense mechanism that escalates the protection for insurers' data collection. The main idea of this mechanism is to augment the insurer's data collection device with the ability to gather unforgeable data acquired from the physical world, and then leverage these data to identify manipulated data points. Our defense mechanism leveraged a statistical model built on unmanipulated data and is robust to manipulation methods that are not foreseen previously. We have implemented this defense mechanism as a proof-of-concept prototype and tested its effectiveness in the real world. Our evaluation shows that our defense mechanism exhibits a false positive rate of 0.032 and a false negative rate of 0.013.

==> dataProcessing.tex <==
\section{Data Representaion \& Processing}


\subsection{}
{[\color{blue} Comment:  In this section, we assume we build a snapshot. The sensors are built in the snapshot. If this is not the case in previous presentation, I will fix it later. I also assume readers have been educated that we use sensor data to verify OBD data]}

\begin{figure}
\centering
\includegraphics[width=0.36\textwidth]{figures/first_ten_second.pdf}
\caption{Example for OBD data and sensor data. [\color{blue} Comment: the figure should be revised to be consistent with other figures; the tiles of the figures should also be changed]}
\label{fig_nvariant}
\end{figure}

{\bf Data Collecting} In our defense prototype, the client is requested to plug in the customized snapshot to the vehicle and make sure the snapshot is firmly attached to the plug-in port. Whenever the client starts the engine, the snapshot activates the built-in sensors and starts requesting data from the OBD interface. Currently we deploy the snapshot with eight sensors,
including an accelerometer. Sampling rates of these sensors are configured to be 200 times per second (the rate reaches the upper limit). From the OBD interface, we request the speed information
and other available information. Initially we set the requesting rate at 20 times per second (the upper limit). However, we observe that the OBD data are updated much less frequently than our sampling. We present an example of the speed series from a ten second trip in the upper half of Figure \ref{fig_nvariant}. In this example, the updating rate is about once per second. In fact, different vehicles may have different updating rates but typically the updating is less frequently than once per second. Therefore, we make the snapshot request OBD data once per second. The collecting will stop as the engine stops.
%The OBD requesting rate is set at 20 times per second (both of the two rates reach the upper limit).
%Note that our calculation method captures any update of speed.


For the simplicity of presentation,
we will use \emph{obd data} to refer to data requested from the OBD interface and \emph{sensor data} to refer to data collected by the sensors. The two types of data
as well as the sampling timestamps are firstly sent to a cell phone via bluetooth and then transformed to a computation server
(in practice, the data should be delivered to a remote server via the 3G channels).


{\bf Data Processing} Now we explain how we process the raw data. In the computation server, we extract the series of speed from the OBD data and the series of three-directional acceleration
from the sensor data. We denote the speed series as a vector $Spe$ and the acceleration series as another vector $Acc$. Each element in $Spe$ records one speed value and the time when the
value is collected ($Spe[i]=(s_{i}, t_{si})$);
Each element in $Acc$ contains values of acceleration in three directions and also the time ($Acc[i]=(ax_{i}, ay_{i}, az_{i}, t_{ai})$).
Basically, the objective of our current defense is to identify in-consistence between $Spe$ and $Acc$.



%However, the OBD data are updated much less frequently than our sampling. We present an example of $Spe$
%from a ten second trip in the upper half of Figure \ref{fig_nvariant}. In this example, the updating rate is about once per %second. Based on our observation, different
%vehicles may have different updating rates but typically the updating is less frequently than once per second. To avoid losing %generality, we calculate the average acceleration
%for each second.

In the first processing phase, we calculate the acceleration series from $Spe$. To get the average acceleration in the $j_{th}$ second, we simply calculate $\frac{s_{i}-s_{i-1}}{ts_{i}-ts_{i-1}}$. Here we use $({ts_{i}-ts_{i-1}})$ as the dividend because the time distance between two samples may slightly deviate from one second. After this process, we turn $Spe$ in to an acceleration
 vector $CAcc$, in which $CAcc[i]$ represents the average acceleration in the $i_{th}$ second. Converting speed into acceleration seems to lose information. However, we have good reasons to do so. On the one hand, the adversaries aim at removing ``hard brakes" from the speed. Based on our observation, the insurance vendors define hard brake as \emph{the speed decreases by a threshold in one second}. So any successful removing of hard brakes will affect how the speed changes as time, which is exactly $CAcc$. On the other hand, the data we use to verify the speed is acceleration from the sensor. What the sensor data can verify is also the changes of speed, namely $CAcc$.

%Intuitively, we can easily get the acceleration at time $ts_{i}$
%via calculating $\frac{s_{i}-s_{i-1}}{ts_{i}-ts_{i-1}}$. To get the average acceleration in the $j_{th}$ second, we first locate %the element $Spe_{p}$ that has time closest to ($ts_{1} + j$) and the element $Spe_{q}$
%that has time closest to ($ts_{1} +j + 1$). Then we take ($Spe{q}-Spe{p}$) as the average acceleration. In this way, we turn %$Spe$ in to an acceleration
% vector $CAcc$, in which $CAcc[i]$ represents the average acceleration in the $i_{th}$ second.

In the second phase, we convert $Acc$ into a vector that also shows the average acceleration in each second. For the $j_{th}$ second, we first identify elements
in $Acc$ that has time falling into $[ta_{1}+j, ta_{1}+j+1)$ and then take the mean of these elements as the average acceleration. Acceleration in different directions are processed separately. We denote the results as $AAcc$, in which $AAcc[i]=(aax_{i}, aay_{i}, aaz_{i})$ represents the average acceleration in three directions during the $i_{th}$ second.

Since the OBD data and the sensor data are collected simultaneously, $CAcc$ and $AAcc$ are time-aligned. In other words, $CAcc[i]$ and $AAcc[i]$ both show the acceleration status
in the $j_{th}$ second. In addition, we multiply each element in $CAcc$ with a constant factor to make them have the same measure as elements in $AAcc$. Our model will take $CAcc$ and $AAcc$ as inputs to detect inconsistence at seconds level, details of which are presented later.

